Indoor positioning systems: Smart fusion of a variety of sensor readings

Robust and versatile localization techniques are key to the success of the next industrial revolution. Yet, it is uncertain which combination of sensors will be the most robust and valuable. Thus, we present a versatile and reproducible measurement system incorporating a manifold number of state-of-the art sensors to compare and fuse the raw input data. It is shown that some techniques show very good results on the same scenario and data-set, but fall apart on translating to a slightly different scenario. In general we show that the vanilla approach to fuse the raw data achieves reasonable results in the generalization domain, demonstrating that radiofrequency (RF) localization techniques in combination with an inertial measurement unit (IMU) could result in a very robust and promising candidate for solving this challenging task.

==> sections/calc.tex <==

\begin{equation}
    r_0^2 = x^2 +y^2 
\end{equation}
\begin{equation}
    r_1^2 = (x-x_1)^2 +(y-y_1)^2 
\end{equation}
\begin{equation}
    r_2^2 = (x-x_2)^2 +(y-y_2)^2 
\end{equation}


\begin{align*}
    r_0^2-  r_2^2 &= x^2 +y^2 - (x-x_2)^2 - (y-y_2)^2 \\               &= x^2+y^2 - (x^2 -2xx_2+x_2^2 ) - (y^2 -2yy_2+y_2^2)\\
                  &= 2xx_2-x_2^2+2yy_2-y_2^2
\end{align*}

\begin{align*}
    2xx_2  &=  r_0^2 -  r_2^2 +x_2^2-2yy_2+y_2^2  \\ 
           x       &= \frac{r_0^2 -r_2^2 +x_2^2-2yy_2+y_2^2}{2x_2}
\end{align*}

\begin{align*}
           x       &= \frac{r_0^2 -r_1^2 +x_1^2-2yy_1+y_1^2}{2x_1}
\end{align*}


\begin{align*}
\frac{r_0^2 -r_2^2 +x_2^2-2yy_2+y_2^2}{2x_2}       &= \frac{r_0^2 -r_1^2 +x_1^2-2yy_1+y_1^2}{2x_1} \\
          (r_0^2 -r_2^2 +x_2^2-2yy_2+y_2^2){2x_1}  &= (r_0^2 -r_1^2 +x_1^2-2yy_1+y_1^2)2x_2
\end{align*}


\begin{align*}
           y       &= \frac{r_0^2 -r_1^2 +x_1^2-2xx_1+y_1^2}{2y_1}\\
           y       &= \frac{r_0^2 -r_2^2 +x_2^2-2xx_2+y_2^2}{2y_2}
\end{align*}

\begin{align*}
         \frac{r_0^2 -r_1^2 +x_1^2-2xx_1+y_1^2}{2y_1}  &= \frac{r_0^2 -r_2^2 +x_2^2-2xx_2+y_2^2}{2y_2} \\
        (r_0^2 -r_1^2 +x_1^2-2xx_1+y_1^2)2y_2  &= (r_0^2 -r_2^2 +x_2^2-2xx_2+y_2^2)2y_1 \\
\end{align*}

\begin{align*}
        r_0^2 y_2 -r_1^2y_2 +y_2x_1^2-y_22xx_1+y_2y_1^2  &= r_0^2y_1 -r_2^2y_1 +y_1x_2^2-y_12xx_2+y_1y_2^2 \\
\end{align*}
\begin{align*}
        2xx_2y_1 -2y_2xx_1  &= r_0^2y_1 -r_2^2y_1 +y_1x_2^2+y_1y_2^2 - r_0^2 y_2 +r_1^2y_2 -y_2x_1^2-y_2y_1^2 \\
\end{align*}
\begin{align*}
        x  &= \frac{r_0^2y_1 -r_2^2y_1 +y_1x_2^2+y_1y_2^2 - r_0^2 y_2 +r_1^2y_2 -y_2x_1^2-y_2y_1^2}{2x_2y_1 -2y_2x_1} \\
\end{align*}

==> tex_content/macros.tex <==
% Vectors
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\vecs}[1]{\boldsymbol{#1}}

\newcommand{\av}{\vec{a}}
\newcommand{\bv}{\vec{b}}
\newcommand{\cv}{\vec{c}}
\newcommand{\dv}{\vec{d}}
\newcommand{\ev}{\vec{e}}
\newcommand{\fv}{\vec{f}}
\newcommand{\gv}{\vec{g}}
\newcommand{\hv}{\vec{h}}
\newcommand{\iv}{\vec{i}}
\newcommand{\jv}{\vec{j}}
\newcommand{\kv}{\vec{k}}
\newcommand{\lv}{\vec{l}}
\newcommand{\mv}{\vec{m}}
\newcommand{\nv}{\vec{n}}
\newcommand{\ov}{\vec{o}}
\newcommand{\pv}{\vec{p}}
\newcommand{\qv}{\vec{q}}
\newcommand{\rv}{\vec{r}}
\newcommand{\sv}{\vec{s}}
\newcommand{\tv}{\vec{t}}
\newcommand{\uv}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\wv}{\vec{w}}
\newcommand{\xv}{\vec{x}}
\newcommand{\yv}{\vec{y}}
\newcommand{\zv}{\vec{z}}
\newcommand{\zerov}{\vec{0}}
\newcommand{\onev}{\vec{1}}
\newcommand{\alphav}{\vecs{\alpha}}
\newcommand{\betav}{\vecs{\beta}}
\newcommand{\gammav}{\vecs{\gamma}}
\newcommand{\lambdav}{\vecs{\lambda}}
\newcommand{\omegav}{\vecs{\omega}}
\newcommand{\sigmav}{\vecs{\sigma}}
\newcommand{\tauv}{\vecs{\tau}}

% Matrices
\newcommand{\Am}{\vec{A}}
\newcommand{\Bm}{\vec{B}}
\newcommand{\Cm}{\vec{C}}
\newcommand{\Dm}{\vec{D}}
\newcommand{\Em}{\vec{E}}
\newcommand{\Fm}{\vec{F}}
\newcommand{\Gm}{\vec{G}}
\newcommand{\Hm}{\vec{H}}
\newcommand{\Id}{\vec{I}}
\newcommand{\Jm}{\vec{J}}
\newcommand{\Km}{\vec{K}}
\newcommand{\Lm}{\vec{L}}
\newcommand{\Mm}{\vec{M}}
\newcommand{\Nm}{\vec{N}}
\newcommand{\Om}{\vec{O}}
\newcommand{\Pm}{\vec{P}}
\newcommand{\Qm}{\vec{Q}}
\newcommand{\Rm}{\vec{R}}
\newcommand{\Sm}{\vec{S}}
\newcommand{\Tm}{\vec{T}}
\newcommand{\Um}{\vec{U}}
\newcommand{\Vm}{\vec{V}}
\newcommand{\Wm}{\vec{W}}
\newcommand{\Xm}{\vec{X}}
\newcommand{\Ym}{\vec{Y}}
\newcommand{\Zm}{\vec{Z}}
\newcommand{\Lambdam}{\vecs{\Lambda}}
\newcommand{\Pim}{\vecs{\Pi}}


% Calligraphic
\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}

\newcommand{\CN}{\Cc\Nc}

% Number sets
\newcommand{\CC}{\mathbb{C}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}

% Mixed symbols
\newcommand{\htp}{^{\mathsf{H}}}
\newcommand{\tp}{^{\mathsf{T}}}


% Brackets
\newcommand{\LB}{\left(}
\newcommand{\RB}{\right)}
\newcommand{\LP}{\left\{}
\newcommand{\RP}{\right\}}
\newcommand{\LSB}{\left[}
\newcommand{\RSB}{\right]}

\renewcommand{\ln}[1]{\mathop{\mathrm{ln}}\LB #1\RB}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\cs}[1]{\mathop{\mathrm{cs}}\LSB #1\RSB}

% Expectation, Variance, etc
\newcommand{\EE}{{\mathbb{E}}}
\newcommand{\Expect}[2]{\EE_{#1}\LSB #2\RSB}

% Theorems, Lemma, etc.
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}



==> tex_content/notations.tex <==
\chapter*{Notations \label{chap:Notations}}

\addcontentsline{toc}{chapter}{Notations}
\markboth{Notations}{Notations}
\setlength\extrarowheight{1em}
\begin{flushleft}
	\begin{longtable}{>{\raggedright}p{0.3\textwidth} >{\raggedright}p{0.69\textwidth}}
	$x$ & scalar variables, especially in time domain: italic lower case letters
	\tabularnewline
	$\mathbf{X}$ & matrix variables: boldface upright upper case letters
	\tabularnewline	
	$x\left(t\right)$ & functions of continuous variables: argument is placed in round parentheses
	\tabularnewline
	$x_{k}$ & scalar elements of a vector or element of a sequence: element index is a subscript
	\tabularnewline
	$X_{ij}$ & scalar elements of a matrix: row and column indices are subscripts
	\tabularnewline
	$\oplus$  & exclusive disjunction (xor)
	\tabularnewline
	$x \ast h $        & convolution of $x$ and $h$
	\tabularnewline
	$P[x<X]$         & probability of $x$ being smaller than $X$
	\tabularnewline
	$\mathbb{E}[X]$         & expected value of $X$
	\tabularnewline
	$\bf{H} \odot \bf{I}$      & Hadamard product of matrix $\bf{H}$ and $\bf{I}$ 
	\tabularnewline
	$j$       & imaginary unit
	\tabularnewline
	$<.>$     & Iverson brackets, turning the statement into Boolean
	\tabularnewline
	$\bf{H}^{\dagger}$ & pseudo inverse of $\bf{H}$
	\end{longtable}
	\par
\end{flushleft}
\setlength\extrarowheight{0em}


==> tex_content/plotcyclelists.tex <==
\pgfplotscreateplotcyclelist{corporate colours markers}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
orange, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
lila, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
hellgrau, mark=text,text mark=p\\%
anthrazit, mark=text,text mark=a\\%
}

\pgfplotscreateplotcyclelist{corporate colours markers double}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
rot, dashed, every mark/.append style={fill=.!80!rot,solid},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
mittelblau, dashed, every mark/.append style={fill=.!80!mittelblau,solid},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
apfelgruen, dashed, every mark/.append style={fill=.!80!apfelgruen,solid},mark=triangle*\\%
orange, mark=star\\%
orange, dashed, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
pink, dashed, every mark/.append style={fill=.!80!pink,solid},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
violettblau, dashed, every mark/.append style={fill=.!80!violettblau,solid},mark=otimes*\\%
lila, mark=|\\%
lila, dashed, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
gelb, dashed, every mark/.append style={fill=.!80!gelb,solid},mark=pentagon*\\%
}
